Formation of C$_{18}$H and C$_{18}$H$_2$ molecules by low energy irradiation with atomic and molecular hydrogen

We study the formation of C$_{18}$H and C$_{18}$H$_2$ by irradiating a cyclo[$18$]carbon molecule with atomic and molecular hydrogen at impact energy, $E$, in the range of 0.5-25 eV. We utilize the density-functional tight-binding method to perform molecular dynamics simulations to emulate the interaction of a carbon ring when colliding with atomic or molecular hydrogen. From our results, the formation of the C$_{18}$H molecules is likely to occur upon irradiating by H atoms at $E < 10$ eV and by H$_2$ molecules at $2 < E < 15$ eV center of mass energy. Formation of C$_{18}$H$_2$ molecules is only observed at around $E = 2$ eV. Our results show that the absorption of hydrogen is more prone in atomic than in molecular hydrogen atmosphere. Thus, we find that the probability of physio-absorption reaches up to 80 \% for atomic projectiles with $E < 5$ eV but only up to 10 \% for the molecular ones. Our analysis shows that the deformation of the carbon ring due to the hydrogen bonding produces transition from $sp$ to $sp^2$ hybridization. The angle between the carbon atoms at the locations near to the H bond in the resulting ring is not 120$^o$ but instead 110$^o$ degrees. No molecular fragmentation of the C$_{18}$ ring is observed.

==> sections/supp_mat.tex <==
We provide the raw data of the potential energy curves obtained by different 
SK parameters for the considered adsorbate cites, that are graphically reported
in Sec 3.1. 
We also include the visualization of the formation of a C$_{18}$H molecule at 
2 eV by using the 3OB SK parameters with DFTD3 dispersion correction, as well as
the four different event observed during the hydrogen irradiation of the C$_{18}$ 
molecule by H$_2$ molecules.
